PIDForest: Anomaly Detection via Partial Identification

We consider the problem of detecting anomalies in a large dataset. We propose a framework called Partial Identification which captures the intuition that anomalies are easy to distinguish from the overwhelming majority of points by relatively few attribute values. Formalizing this intuition, we propose a geometric anomaly measure for a point that we call PIDScore, which measures the minimum density of data points over all subcubes containing the point. We present PIDForest: a random forest based algorithm that finds anomalies based on this definition. We show that it performs favorably in comparison to several popular anomaly detection methods, across a broad range of benchmarks. PIDForest also provides a succinct explanation for why a point is labelled anomalous, by providing a set of features and ranges for them which are relatively uncommon in the dataset.

==> exact.tex <==
\section{An algorithm to compute $\pidsc$}

It appears that any algorithm for computing $\pidsc$ exactly will depend exponentially in
$d$. However, it leaves open to possibility of computing it
efficiently in low dimensions, for instance when $d =1$.
Below we restate the problem for $1$ dimension:

{\bf 1-dimensional $\pidsc$:} Given $\T = \{ x_1, \ldots,
x_n\} \in \intzo$ where $x_i$s are sorted, for each $j \in [n]$,
find the interval $I \subseteq \intzo$ containing $j$ such that
$\rho(I) = \len(I)/|T \cap I|$ is minimized.

To simplify matters, we restrict to those intervals whose start and end points of the
are either $e_0 = 0$, $e_n =1$, or $e_i = (x_i +x_{i+1})/2$ for $i \in
[n-1]$. Observe that the $e_i$s interleave with the $x_j$s.
For $1 \leq \ell \leq u \leq n$, let $E_{\ell,u}$ denote the
continuous interval $[e_{\ell -1}, e_u]$, note that it contains points $\{x_\ell, \ldots, x_u\}$.
We restrict ourselves to minimizing these intervals.
This avoids issues that might arise from the precision of the end
points, and reduces the search space of intervals to $O(n^2)$. This
implies in a trivial $O(n^3)$ algorithm, where for each point, we
consider all intervals that contain it. Our main theoretical
contribution is a linear time algorithm to compute $\pid$ in dimension
$1$.

For $\ell, u \in [n]$, where $\ell \leq u$ let $I_\ell^u = \{\ell,
\cdots, u\}$ denote the discrete interval. The first step is to reduce
the problem to the {\em densest interval} problem for arrays:

{\bf Densest interval:} Given values $(a_1, \ldots, a_n) \in \R$,
for each $j \in [n]$, find the interval $I_\ell^u$ which maximizes
\[ \rho(I_\ell^u) = \frac{\sum_{j = \ell}^u a_j}{(u - \ell + 1)}. \]

To reduce from 1-d $\pidsc$ to Densest interval,
we assign to each point the interval around it: for $i \in [n]$, let
$a_i = \len(E_{i, i}) =  e_i - e_{i-1}$ be its length. It follows that
\[ \rho(I_\ell^u) = \frac{\sum_{j = \ell}^u a_j}{(u - \ell + 1)} = \frac{(e_u
- e_{\ell -1})}{u - (\ell - 1)} = \rho(E_{\ell, u}).\]

We present a linear time algorithm for densest interval in Appendix \ref{app:dense}.

